Analyzing and Simulating User Utterance Reformulation in Conversational Recommender Systems

User simulation has been a cost-effective technique for evaluating conversational recommender systems. However, building a human-like simulator is still an open challenge. In this work, we focus on how users reformulate their utterances when a conversational agent fails to understand them. First, we perform a user study, involving five conversational agents across different domains, to identify common reformulation types and their transition relationships. A common pattern that emerges is that persistent users would first try to rephrase, then simplify, before giving up. Next, to incorporate the observed reformulation behavior in a user simulator, we introduce the task of reformulation sequence generation: to generate a sequence of reformulated utterances with a given intent (rephrase or simplify). We develop methods by extending transformer models guided by the reformulation type and perform further filtering based on estimated reading difficulty. We demonstrate the effectiveness of our approach using both automatic and human evaluation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> RQ2_table.tex <==
\begin{table}[t]
\footnotesize
    \centering
        \caption{The mutual information between user's experience and reformulation type in different agent}
        \captionshrink
    \begin{tabular}{c|ccccc}
    \toprule
      \textbf{Agent} & A1 & A2 & A3 & A4 & A5 \\
      \midrule
    \textbf{mutual info} & 0.046 & 0.032 & 0.028 & 0.024 & 0.019 \\
    \bottomrule
    \end{tabular}
    \label{tbl:RQ2}
    \captionshrink
\end{table}

==> RQ2_ttest.tex <==
\begin{table}[t]
\footnotesize
    \centering
        \caption{Significance test between users with and without experience of conversational \sz{agents}.}
        % \todo{agents/recommenders}.}
        \captionshrink
    \begin{tabular}{c|cccccc}
    \toprule
      \textbf{Type} & Restart & Repeat & Rephrase & Simplify & Refine & Stop \\
      \midrule
    \textbf{p-value} & 0.685 & 0.734 & 0.578 & 0.264 & 0.154 & 0.646  \\
    \bottomrule
    \end{tabular}
    \label{tbl:RQ2-ttest}
    \captionshrink
\end{table}

==> RQ3_table.tex <==
\begin{table}[t]
\footnotesize
    \centering
        \caption{The stationary dist(ribution) of reformulation types.}
        \captionshrink
    \begin{tabular}{c|ccccccc}
    \toprule
      \textbf{Type} & Restart & Repeat & Rephrase & Simplify & Refine & Change & Stop \\
      \midrule
    \textbf{Dist} & 0.23 & 0.03 & 0.16 & 0.09 & 0.07 & 0.31 & 0.11\\
    \bottomrule
    \end{tabular}
    \label{tbl:RQ3}
    \captionshrink
\end{table}

==> anaysis_table.tex <==
%
\begin{table}[t]
	\caption{Classification of comments accompanying decisions when choosing which of two conversations was made by a real user versus a simulated one in a side-by-side comparison.  The columns are (Rea)listicity, (Eng)agement, (Emo)tion, (Res)ponse, (Gra)mmar, and (Len)gth.}
% 	\captionshrink	
	\begin{tabular}{lrrrlrrr}
	\toprule
	& \multicolumn{3}{c}{\textbf{Style}} && \multicolumn{3}{c}{\textbf{Content}} \\ 
	\cline{2-4} 	\cline{6-8}
	 &\textbf{Rea.} & \textbf{Eng.} & \textbf{Emo.} && 
	 \textbf{Res.} & \textbf{Gra.} & \textbf{Len.} \\
	\midrule
	Method 1 & 
		- & - & - && 
		- & - & -  \\
	Method 2 & 
		- & - & - && 
		- & - & -  \\
	Method 3 & 
		- & - & - && 
		- & - & -  \\
	\midrule
	All & 
		- & - & - && 
		- & - & - \\
	\bottomrule
	\end{tabular}
% 	\shrink
\label{tbl:anay}
\vspace*{-0.75\baselineskip}
\end{table}
%
